Fundamental Limitations within the Selected Cryptographic Scenarios and Supra-Quantum Theories

The following submission constitutes a guide and an introduction to a collection of articles submitted as a Ph.D. dissertation at the University of Gda\'nsk. In the dissertation, we study the fundamental limitations within the selected quantum and supra-quantum cryptographic scenarios in the form of upper bounds on the achievable key rates. We investigate various security paradigms, bipartite and multipartite settings, as well as single-shot and asymptotic regimes. Our studies, however, extend beyond the derivations of the upper bounds on the secret key rates in the mentioned scenarios. In particular, we propose a novel type of rerouting attack on the quantum Internet for which we find a countermeasure and benchmark its efficiency. Furthermore, we propose several upper bounds on the performance of quantum (key) repeaters settings. We derive a lower bound on the secret key agreement capacity of a quantum network, which we tighten in an important case of a bidirectional quantum network. The squashed nonlocality derived here as an upper bound on the secret key rate is a novel non-faithful measure of nonlocality. Furthermore, the notion of the non-signaling complete extension arising from the complete extension postulate as a counterpart of purification of a quantum state allows us to study analogies between non-signaling and quantum key distribution scenarios.

==> arXiv_abstract.tex <==






The following submission constitutes a guide and an introduction to a collection of articles submitted as a Ph.D. dissertation at the University of Gda{\' n}sk. In the dissertation, we study the fundamental limitations within the selected quantum and supra-quantum cryptographic scenarios in the form of upper bounds on the achievable key rates. We investigate various security paradigms, bipartite and multipartite settings, as well as single-shot and asymptotic regimes. Our studies, however, extend beyond the derivations of the upper bounds on the secret key rates in the mentioned scenarios. In particular, we propose a novel type of rerouting attack on the quantum Internet for which we find a countermeasure and benchmark its efficiency. Furthermore, we propose several upper bounds on the performance of quantum (key) repeaters settings. We derive a lower bound on the secret key agreement capacity of a quantum network, which we tighten in an important case of a bidirectional quantum network. The squashed nonlocality derived here as an upper bound on the secret key rate is a novel non-faithful measure of nonlocality. Furthermore, the notion of the non-signaling complete extension arising from the complete extension postulate as a counterpart of purification of a quantum state allows us to study analogies between non-signaling and quantum key distribution scenarios. 

% In the collection of articles constituting this dissertation, of which I am a coauthor, as our primary interest, we study the fundamental limitations within the selected quantum and supra-quantum cryptographic scenarios in the form of upper bounds on the achievable key rates.  Specifically, our findings contribute to the secret key agreement scenario (SKA), device-dependent conference key agreement scenario (DD-CKA) both for quantum channels and quantum states in one-shot and asymptotic regimes, device-independent conference key-agreement scenario (DI-CKA) in both asymptotic and one-shot regime, and non-signaling device-independent secret key agreement scenario (NSDI). Our studies, however, extend beyond the derivations of the upper bounds on the secret key rates in the mentioned scenarios. In particular, we propose a novel type of rerouting attack on the quantum Internet for which we find a countermeasure and benchmark its efficiency. Furthermore, we propose several upper bounds on the performance of quantum (key) repeaters settings. We derive a lower bound on the secret key agreement capacity of a quantum network, which we tighten in an important case of a bidirectional quantum network. The squashed nonlocality derived here as an upper bound on the secret key rate is a novel non-faithful measure of nonlocality. Furthermore, the notion of the non-signaling complete extension arising from the complete extension postulate as a counterpart of purification of a quantum state allows us to study analogies between non-signaling and quantum key distribution (QKD) scenarios. 





==> frontmatter/declaration.tex <==
%
% File: declaration.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the declaration page
%
% UoB guidelines:
%
% Author's declaration
%
% I declare that the work in this dissertation was carried out in accordance
% with the requirements of the University's Regulations and Code of Practice
% for Research Degree Programmes and that it has not been submitted for any
% other academic award. Except where indicated by specific reference in the
% text, the work is the candidate's own work. Work done in collaboration with,
% or with the assistance of, others, is indicated as such. Any views expressed
% in the dissertation are those of the author.
%
% SIGNED: .............................................................
% DATE:..........................
%
\chapter*{Author's declaration}
\begin{SingleSpace}
\begin{quote}
\initial{I} declare that the work in this dissertation was carried out in accordance with the requirements of  the University's Regulations and Code of Practice for Research Degree Programmes and that it  has not been submitted for any other academic award. Except where indicated by specific  reference in the text, the work is the candidate's own work. Work done in collaboration with, or with the assistance of, others, is indicated as such. Any views expressed in the dissertation are those of the author.

\vspace{1.5cm}
\noindent
\hspace{-0.75cm}\textsc{SIGNED: .................................................... DATE: ..........................................}
\end{quote}
\end{SingleSpace}
\clearpage
